Distributed Sparse Feature Selection in Communication-Restricted Networks

This paper aims to propose and theoretically analyze a new distributed scheme for sparse linear regression and feature selection. The primary goal is to learn the few causal features of a high-dimensional dataset based on noisy observations from an unknown sparse linear model. However, the presumed training set which includes $n$ data samples in $\mathbb{R}^p$ is already distributed over a large network with $N$ clients connected through extremely low-bandwidth links. Also, we consider the asymptotic configuration of $1\ll N\ll n\ll p$. In order to infer the causal dimensions from the whole dataset, we propose a simple, yet effective method for information sharing in the network. In this regard, we theoretically show that the true causal features can be reliably recovered with negligible bandwidth usage of $O\left(N\log p\right)$ across the network. This yields a significantly lower communication cost in comparison with the trivial case of transmitting all the samples to a single node (centralized scenario), which requires $O\left(np\right)$ transmissions. Even more sophisticated schemes such as ADMM still have a communication complexity of $O\left(Np\right)$. Surprisingly, our sample complexity bound is proved to be the same (up to a constant factor) as the optimal centralized approach for a fixed performance measure in each node, while that of a na\"{i}ve decentralized technique grows linearly with $N$. Theoretical guarantees in this paper are based on the recent analytic framework of debiased LASSO in Javanmard et al. (2019), and are supported by several computer experiments performed on both synthetic and real-world datasets.

==> README <==
********************************************************************
   ASME DETC LaTeX Style for LaTeX verson 2e
********************************************************************

********************************************************************
Release history: 
   version 1.7, August 1, 2012. 
      (1) added 
       \special{papersize=8.5in,11in}
        to asme2e.tex
                       --- Hongtai Cheng <h_c45@txstate.edu>
   version 1.7, Jan 11, 2010. 
      Modified asme2e.cls with the following changes:
       (1) Greek letters in math mode are italicized.
       (2) Figure captions are in uppercase bold sans serif font of 9 points.
       (3) The defined commands \hour \minute conflict with the commands 
           \hour and minute in the approved package SIunits.  
           They were changed to \thour and \tminute.
                          --- Marc LaViolette <laviolette-m@rmc.ca>
   version 1.6, May 24, 2009. 
       (1) Modified asmems4.bst to use \textbf for handling boldface.
                          --- Tim Lahey <tjlahey@cgl.uwaterloo.ca>
   version 1.5, January 12, 2009. 
       (1) Modified asme2e.tex to use a new header
       (2) Modified asme2e.cls to use a new header
                          --- Harry H. Cheng hhcheng@ucdavis.edu
   version 1.4, May 12, 2005. 
       (1) Modified asme2e.cls to support pdflatex  
       (2) Modified asme2e.cls to support multiple lines in conference name.
           asme2e.tex modified with a conference with multiple lines.
                          --- Matt Campbell matthew.campbell@goodrich.com
   version 1.3, Januaray 9, 2005. 
       (1) Top margin of the layput changed in asme2e.cls.
       asme2e.cls1.2 is for ASME DETC template version 1.2.

       (2) Updated asmms4.bst to conform the ASME reference format.
       It fixes 2 items in the article format: 1) a extraneous space 
       after number or month was removed, and 2) an incorrect font style 
       that occurred for one particular combination of number 
       and month data was corrected. It also adjusts capitalization 
       in proceedings entries to correspond to the latest ASME reference 
       format. The current ASME reference format still does not 
       completely resolve all formatting issues. In particular, 
       the sample bibliography uses roman style for journal names  
       in an article citation, but the reference format doesn't 
       actually specify a style for the journal name. Since there's 
       some ambiguity here, I left the journal name italicized.
                          --- Geoffrey Shiflett shiflett@usc.edu          

   version 1.2, August 28, 2003. 
       updated asme2e.cls. The 1st page heading is
       location, date instead of the reverse.
   version 1.2, August 26, 2003. 
       updated ASME bibliography style file asmems4.bst.
       removed brackets surrounding month in article citations
   version 1.2, January 25, 2003. 
       support the modified ASME bibliography style
   version 1.1, February 16, 2001 
       support new ASME bibliography style
   No version num, May 7, 1994
       the initial distribution of the template

********************************************************************
Files included in this distribution:

FAQ            frequently asked questions.
README         this file
README2        information about  Postscript Type 1 fonts
               if you run into trouble with times.sty, mathptm.sty,
               and pifont.sty.
Makefile       a sample Makefile for creating asme2e.pdf and 
               abstract.pdf in Unix.
asme2e.cls     LaTeX style class package for papers of the American
               Society of Mechanical Engineers. Questions related to
               asme2e.cls may be addressed to Ken Sprott 
               at sprottk@gaia.ecs.csus.edu
asmems4.bst    ASME bibliography style file. Questions related to
               asmems4.bst may be addressed to Geoffrey Shiflett 
               at shiflett@usc.edu          
asme2e.tex     Sample file which uses the asme2e.cls and documents 
               some specifications of ASME paper.
asme2e.pdf     PDF file generated from asme2e.tex
asbstract.tex  Template of the extended abstract of an ASME paper.
asbstract.pdf  PDF file generated from abstract.tex.


********************************************************************
Note: (1) To get article asme2e in TeX dvi format, type
             latex asme2e
             bibtex asme2e
             latex asme2e
             dvips -o asme2e.ps asme2e
      (2) To get asmee2.pdf file from TeX dvi file, use Adobe Acrobat or type
             ps2pdf asme2e.ps asme2e.pdf
      (2) The package array is included in the class file asme2e.cls. 
          See "The LaTeX Companion" book for a description of its use 
          in compiling tables.
      (3) The class file asme2e.cls will not produce unnumbered theorems 
          in the theorem environment.
      (4) To get unnumbered equations, use the package amslatex
          in your document.

********************************************************************
Contributors:
   Harry H. Cheng    hhcheng@ucdavis.edu     
           the original creator of the template.
   Kirk Van Katwyk   
           contributed to asme.sty and asme2e.cls
   Ken Sprott        sprottk@gaia.ecs.csus.edu
           contributed asme2e.cls and ASME bibliography 
   Geoffrey Shiflett shiflett@usc.edu          
           created ASME bibliography stype file asmems4.bst with details 
           explained in asme2e.tex.
   Matt Campbell matthew.campbell@goodrich.com
           modified asme2e.cls to support pdflatex and conference name with
           multiple lines.


